The Cuntz-Pimsner algebra of the simplest Motzkin subproduct system is 2-subhomogeneous

The Motzkin subproduct system (SPS) is constructed from the Jones Wenzl idempotents of the Motzkin algebras, which generalizes the Temperley Lieb SPS. The simplest Motzkin SPS, which is not a Temperley Lieb SPS, is constructed from a 3 dimensional Hilbert space. We explicitly describe the spectrum of the corresponding Cuntz Pimsner algebra, which remarkably admits only irreducible representations of dimensions 1 and 2, and can thus be viewed as a mildly quantum space. We moreover analyse representations of the Richard Thompson groups and of the Cuntz algebra that are associated to this spectrum.

==> bib.tex <==

%%\begin{bibdiv}
%\begin{biblist}
 
\bib{ALV}{article}{
  title={Interacting Fock spaces and Hilbert module extensions of the Heisenberg commutation relations},
  author={Accardi, Luigi},
  author={Lu, Yun-Gang},
  author={Volovich, Igor},
  journal={Publications of IIAS, Kyoto},
  year={1997},
}

 


\bib{ACRsurvey}{article}{
  title={A hitchhiker’s guide to endomorphisms and automorphisms of Cuntz algebras},
author={Aiello, Valeriano},
  author={Conti, Roberto},
  author={Rossi, Stefano},
    journal={Rend. Mat. Appl},
  volume={42},
  pages={61--162},
  year={2021},
}

 

\bib{ADR01}{article}{
  title={The Motzkin subproduct system},
author={Aiello, Valeriano},
  author={Del Vecchio, Simone},
  author={Rossi, Stefano}, 
  journal={International Journal of Mathematics},
  volume={36},
  number={14},
  pages={2550060},
  year={2025},
  publisher={World Scientific},
  note={preprint \href{https://arxiv.org/abs/2502.14057}{arXiv:2502.14057}},
}

 


\bib{AK}{article}{
  title={Gysin sequences and $SU(2)$-symmetries of C$^*$-algebras},
  author={Arici, Francesca},
  author={Kaad, Jens},
  journal={Transactions of the London Mathematical Society},
  volume={8},
  number={1},
  pages={440--492},
  year={2021},
  publisher={Wiley Online Library},
}

\bib{Nesh3}{article}{
  title={KK-duality for the Cuntz-Pimsner algebras of Temperley-Lieb subproduct systems},
  author={Arici, Francesca},
  author={Gerontogiannis, Dimitris},
  author={Neshveyev, Sergey},
  journal={preprint arXiv:2401.01725},
  year={2024},
}



\bib{Arveson98}{article}{
 Author = {Arveson, William},
 Title = {Subalgebras of C$^*$-algebras. III: Multivariable operator theory},
 %FJournal = {Acta Mathematica},
 Journal = {Acta Math.},
 %ISSN = {0001-5962},
 Volume = {181},
 Number = {2},
 Pages = {159--228},
 Year = {1998},
 %Language = {English},
 DOI = {10.1007/BF02392585},
 %Keywords = {46L05,47L80},
% zbMATH = {1269879},
% Zbl = {0952.46035}
}
 

\bib{Bhat}{article}{ 
  title={Inclusion systems and amalgamated products of product systems},
  author={Bhat, BV Rajarama},
  author={Mukherjee, Mithun},
  journal={Infinite Dimensional Analysis, Quantum Probability and Related Topics},
  volume={13},
  number={01},
  pages={1--26},
  year={2010},
  publisher={World Scientific},
}
 
\bib{Halverson}{article}{
  title={Motzkin algebras},
  author={Benkart, Georgia},
  author={Halverson, Tom},
  journal={European Journal of Combinatorics},
  volume={36},
  pages={473--502},
  year={2014},
  publisher={Elsevier},
}

\bib{Birget03}{article}{ 
  title={The groups of Richard Thompson and complexity},
  author={Birget, Jean-Camille},
  journal={International Journal of Algebra and Computation},
  volume={14},
  number={05n06},
  pages={569--626},
  year={2004},
  publisher={World Scientific}
}

 
\bib{Brothier-Jones19}{article}{
AUTHOR = {Brothier, Arnaud},
AUTHOR = {Jones, Vaughan F. R.},
TITLE = {Pythagorean representations of Thompson's groups},
JOURNAL = {J. Funct. Anal.},
FJOURNAL = {Journal of Functional Analysis},
VOLUME = {277},
YEAR = {2019},
NUMBER = {7},
PAGES = {2442--2469},
ISSN = {0022-1236},
MRCLASS = {22D25 (20F65 46L05)},
MRNUMBER = {3989149},
MRREVIEWER = {Bachir Bekka},
DOI = {10.1016/j.jfa.2019.02.009},
URL = {https://doi-org.proxy.library.vanderbilt.edu/10.1016/j.jfa.2019.02.009},
}
		
 

\bib{Brothier-Wijesena25}{article}{
title={Jones' representations of R. Thompson's groups not induced by finite-dimensional ones},
author={Brothier, Arnaud},
author={Wijesena, Dilshan},
journal={Annales de l'Institut Fourier},
volume={75},
issue={6},
pages={2677-2716}, 
year={2025},
}

\bib{Brothier-Wijesena26}{article}{
title={Atomic representations of R.~Thompson's groups and
Cuntz's algebra},
author={Brothier, Arnaud},
author={Wijesena, Dilshan},
journal={Documenta Mathematica},
volume={31},
issue={2},
pages={355-383}, 
year={2026},
}

\bib{Brothier-Wijesena24}{article}{
  title={Irreducible Pythagorean representations of R. Thompson's groups and of the Cuntz algebra},
author={Brothier, Arnaud},
author={Wijesena, Dilshan},  
journal={Advances in Mathematics},
  volume={454},
  pages={109871},
  year={2024},
  publisher={Elsevier},
}

 
 
\bib{CFP}{article}{ 
  title={Introductory notes on Richard Thompson’s groups},
  author={Cannon, James W},
  author={Floyd, William J},
  author={Parry, Walter R},
  journal={Enseign. Math.(2)},
  volume={42},
  number={3-4},
  pages={215},
  year={1996}
}


\bib{Cuntz}{article}{ 
title={Simple C$^*$-algebra generated by isometries},
author={Cuntz, Joachim},
journal={Communications in mathematical physics},
volume={57},
number={2},
pages={173--185},
year={1977},
publisher={Springer},
}


\bib{Dixmier64}{article}{
title={Traces sur les C*-alg\`ebres. II},
author={Dixmier, Jacques},
journal={Bull. Sci. Math.},
volume={88},
issue={2},
pages={39-57},
year={1964},
}

\bib{Dixmier}{book}{
  title={C$^*$-Algebras},
  author={Dixmier, Jacques},
  journal={North-Holland Math. Library},
  volume={15},
  year={1977},
  publisher={North-Holland},
}



\bib{DM}{article}{
AUTHOR = {Dudko, Artem},
AUTHOR = {Medynets, Konstantin},
TITLE = {Finite factor representations of Higman-Thompson groups},
JOURNAL = {Groups Geom. Dyn.},
FJOURNAL = {Groups, Geometry, and Dynamics},
VOLUME = {8},
YEAR = {2014},
NUMBER = {2},
PAGES = {375--389},
ISSN = {1661-7207},
MRCLASS = {20C15 (22F10 37A05)},
MRNUMBER = {3231220},
MRREVIEWER = {Nhan-Phu Chung},
DOI = {10.4171/GGD/230},
URL = {https://doi-org.proxy.library.vanderbilt.edu/10.4171/GGD/230},
}

\bib{Garncarek12}{article}{ 
  title={Analogs of Principal Series Representations for Thompson's Groups F and T},
  author={Garncarek, {\L}ukasz},
  journal={Indiana University Mathematics Journal},
  pages={619--626},
  year={2012},
  publisher={JSTOR}
}


\bib{GerholdSkeide}{article}{
  title={Interacting Fock spaces and subproduct systems},
  author={Gerhold, Malte},
  author={Skeide, Michael},
  journal={Infinite Dimensional Analysis, Quantum Probability and Related Topics},
  volume={23},
  number={03},
  pages={2050017},
  year={2020},
  publisher={World Scientific},
}	 

\bib{Halmos69}{article}{ 
  title={Two subspaces},
  author={Halmos, Paul R.},
  journal={Transactions of the American Mathematical Society},
  volume={144},
  pages={381--389},
  year={1969},
  publisher={JSTOR},
}


\bib{Nesh}{article}{
  title={Subproduct systems with quantum group symmetry},
  author={Habbestad, Erik},
  author={Neshveyev, Sergey},
  journal={Journal of Noncommutative Geometry},
  volume={18},
  number={1},
  pages={93--121},
  year={2023},
}
\bib{Nesh2}{article}{
  title={Subproduct systems with quantum group symmetry II},
  author={Habbestad, Erik},
  author={Neshveyev, Sergey},
    journal={Trans. Amer. Math. Soc.},
      volume={378},
   pages={5159-5185},
  year={2025}, 
%  journal={preprint arXiv:2212.08512},
}



\bib{Ly}{article}{
  title={Presentation of the Motzkin monoid},
  author={Hatch, Kris},
  author={Ly, Megan},
    author={Posner, Eliezer},
  journal={preprint arXiv:1301.4518},
  year={2013},
}

\bib{Jones83}{article}{
  title={Index for subfactors},
  author={Jones, Vaughan F.R.},
  journal={Inventiones mathematicae},
  volume={72},
    pages={1--25},
  year={1983}
}

\bib{Jo14}{article}{
  title={Some unitary representations of Thompson’s groups F and T},
AUTHOR = {Jones, Vaughan F.R.},
  journal={J. Comb. Algebra},
  volume={1},
  number={1},
  pages={1--44},
  year={2017}
}

 
\bib{jo2}{article}{
AUTHOR = {Jones, Vaughan F.R.},
title={Planar Algebras I},
journal={New Zealand Journal of Mathematics},
volume={52},
pages={1-107},
note={preprint \href{http://arxiv.org/abs/9909027}{arXiv:9909027}},
year={2021},
}
 

\bib{Jo21}{article}{
  title={Motzkin algebras and the $A_n$ tensor categories of bimodules},
  author={Jones, Vaughan F.R.},
  author={Yang, Jun},
  journal={International Journal of Mathematics},
  volume={32},
  number={10},
  pages={2150077},
  year={2021},
  publisher={World Scientific},
}

\bib{Nekrashevych03}{article}{ 
  title={Cuntz-Pimsner algebras of group actions},
  author={Nekrashevych, Volodymyr V},
  journal={Journal of Operator Theory},
  pages={223--249},
  year={2004},
  publisher={JSTOR}
}



\bib{Pedersen}{book}{ 
  title={Analysis now},
  author={Pedersen, Gert K},
  year={2012},
  publisher={Springer Science \& Business Media}
}  
		
\bib{Popescu}{article}{
  title={Operator theory on noncommutative varieties},
  author={Popescu, Gelu},
  journal={Indiana University mathematics journal},
  pages={389--442},
  year={2006},
  publisher={JSTOR}
}

\bib{Popescu2}{article}{
  title={Operator theory on noncommutative varieties, II},
  author={Popescu, Gelu},
  journal={Proceedings of the American Mathematical Society},
  volume={135},
  number={7},
  pages={2151--2164},
  year={2007}
}
		
		 

\bib{Shalit}{article}{
  title={Subproduct systems},
  author={Shalit, Orr},
  author={Solel, Baruch},
  journal={Documenta Mathematica},
  volume={14},
  pages={801--868},
  year={2009},
}
	
	
	
\bib{Skeide}{article}{
title={Algebraic central limit theorems: A personal view on one of Wilhelm’s legacies},
author={Skeide, Michael},
journal={Infinite Dimensional Analysis, Quantum Probability and Related Topics},
volume={25},
number={04},
pages={2240003},
year={2022},
publisher={World Scientific}, 
}
 

\bib{Viselter12}{article}{ 
  title={Cuntz-Pimsner algebras for subproduct systems},
  author={Viselter, Ami},
  journal={International Journal of Mathematics},
  volume={23},
  number={08},
  pages={1250081},
  year={2012},
  publisher={World Scientific}
}
	
	 
%\end{biblist}
%%\end{bibdiv}
